A Large-Scale Outdoor Multi-modal Dataset and Benchmark for Novel View Synthesis and Implicit Scene Reconstruction

Neural Radiance Fields (NeRF) has achieved impressive results in single object scene reconstruction and novel view synthesis, which have been demonstrated on many single modality and single object focused indoor scene datasets like DTU, BMVS, and NeRF Synthetic.However, the study of NeRF on large-scale outdoor scene reconstruction is still limited, as there is no unified outdoor scene dataset for large-scale NeRF evaluation due to expensive data acquisition and calibration costs. In this paper, we propose a large-scale outdoor multi-modal dataset, OMMO dataset, containing complex land objects and scenes with calibrated images, point clouds and prompt annotations. Meanwhile, a new benchmark for several outdoor NeRF-based tasks is established, such as novel view synthesis, surface reconstruction, and multi-modal NeRF. To create the dataset, we capture and collect a large number of real fly-view videos and select high-quality and high-resolution clips from them. Then we design a quality review module to refine images, remove low-quality frames and fail-to-calibrate scenes through a learning-based automatic evaluation plus manual review. Finally, a number of volunteers are employed to add the text descriptions for each scene and key-frame to meet the potential multi-modal requirements in the future. Compared with existing NeRF datasets, our dataset contains abundant real-world urban and natural scenes with various scales, camera trajectories, and lighting conditions. Experiments show that our dataset can benchmark most state-of-the-art NeRF methods on different tasks. We will release the dataset and model weights very soon.

==> comments_tool/macros.tex <==
% \usepackage{wrapfig}
\usepackage{hyphenat}
\usepackage{soul,color}
\usepackage{amsopn}
% \usepackage{subfigure}
% \usepackage{url}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\itemnudege}{\vspace{-.05in}}
\newcommand{\eqnbreak}{\par\vspace{-1.5\baselineskip}}
\newcommand{\vnudge}{\vspace{-.15in}}

\definecolor{Red}{cmyk}{0,1,1,0}
\definecolor{Green}{cmyk}{1,0,1,0}
\definecolor{Cyan}{cmyk}{1,0,0,0}
\definecolor{Purple}{cmyk}{0.45,0.86,0,0}
\definecolor{Rosolic}{cmyk}{0.00,1.00,0.50,0}
\definecolor{Blue}{cmyk}{1.00,1.00,0.00,0}
\definecolor{BlueViolet}{cmyk}{0.86,0.91,0,0.04}
\definecolor{NavyBlue}{cmyk}{0.94,0.54,0,0}
% \newcommand{\cx}[1]{{\color{Black} #1}}
% \newcommand{\fk}[1]{{\color{Black} #1}}
% \newcommand{\cs}[1]{{\color{Black} #1}}

% \newcommand{\other}[1]{{\color{Rosolic}  Other: #1}}
% \newcommand{\tmp}[1]{{\color{Purple}  Tmp: #1}}

% \newcommand{\cx}[1]{{\color{BlueViolet} cx: #1}}
% \newcommand{\fk}[1]{{\color{Green} fk: #1}}
% \newcommand{\cs}[1]{{\color{Purple} cs: #1}}

\newcommand{\other}[1]{{\color{Black} #1}}
\newcommand{\tmp}[1]{{\color{Black} #1}}

\newcommand{\cx}[1]{{\color{Black} #1}}
\newcommand{\fk}[1]{{\color{Green} #1}}
\newcommand{\cs}[1]{{\color{Black} #1}}

% \newcommand{\maNote}[1]{}
% \newcommand{\chen}[1]{#1}
% \newcommand{\pang}[1]{#1}
% \newcommand{\ma}[1]{#1}


\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{rem}[thm]{Remark}
\let\vec=\mathbf
\let\set=\mathcal
\let\mat=\mathbf

%\newcommand{\mypara}{\subsection}
\newcommand{\mypara}[1]{\paragraph*{#1.}}
\newcommand{\bv}[1]{\mathbf{#1}}
\newcommand{\vv}[1]{\mathbf{#1}}
\newcommand{\todo}[1]{\hl{#1}}
\newcommand{\bi}[1]{\mathbf{#1}}

